A Game-Theoretic Analysis of the Empirical Revenue Maximization Algorithm with Endogenous Sampling

The Empirical Revenue Maximization (ERM) is one of the most important price learning algorithms in auction design: as the literature shows it can learn approximately optimal reserve prices for revenue-maximizing auctioneers in both repeated auctions and uniform-price auctions. However, in these applications the agents who provide inputs to ERM have incentives to manipulate the inputs to lower the outputted price. We generalize the definition of an incentive-awareness measure proposed by Lavi et al (2019), to quantify the reduction of ERM's outputted price due to a change of $m\ge 1$ out of $N$ input samples, and provide specific convergence rates of this measure to zero as $N$ goes to infinity for different types of input distributions. By adopting this measure, we construct an efficient, approximately incentive-compatible, and revenue-optimal learning algorithm using ERM in repeated auctions against non-myopic bidders, and show approximate group incentive-compatibility in uniform-price auctions.

==> changes_summary.tex <==
Our paper was submitted to EC'20 previously.  The EC reviewers were interested in our attempt to introduce incentive-compatible issues to the learning process and like the definition of incentive-awareness measure.  They thought it is nice that guarded-ERM algorithm is not sensitive to strategic bidding.  However, they also pointed out some shortcomings of our previous version:

1. We assumed that buyers' values are i.i.d., which they thought is restricted.

2. We didn't compare our results with other works on repeated auctions against non-myopic bidders. 

3. We didn't discuss the difficulty in our proof of the main theorem.

Changes: We add justifications and discussions for above three points.  We also re-structure the paper so that the incentive-awareness measure instead of the two-phase model becomes the main model, because we think the incentive-awareness measure is more interesting, fundamental, and useful than the two-phase model. 



\section*{Changes of Previous Version}
Our paper was submitted to EC'20 previously. The EC reviewers were interested in our attempt to introduce incentive-compatible issues to the learning process and like the definition of incentive-awareness measure. They thought it is nice that guarded-ERM algorithm is not sensitive to strategic bidding. However, they also pointed out some shortcomings of our previous version:

1. We assumed that buyers' values are i.i.d., which they thought is restricted.

2. We lack some comparisons between our results and some in literature, especially with \citet{liu2018learning}, which use the technique of differential privacy to cope with the problem of learning reserve price in repeated auctions against non-myopic bidders.

3. We do not emphasize the difficulty in our proof of main theorem.


==> delta_centered_intro.tex <==
% \new{we need to shorten the intro, and justify iid setting and the study of ERM}

In auction theory, it is well-known since \citet{myerson1981optimal} that, when all buyers have values that are independently and identically drawn from a regular distribution $F$, the revenue-maximizing auction is simply the second price auction with anonymous reserve price $p^*=\argmax\{p(1-F(p)\}$: if the highest bid is at least $p^*$, then that bidder wins the item and pays the maximium between the second highest bid and $p^*$. 
The computation of $p^*$ requires the exact knowledge of the underlying value distribution $F$, which is an unrealistic requirement because the value distribution is often unavailable in practice.  Many works (e.g., \cite{cole2014the, dhangwatnotai2015revenue, huang2018making}) on sample complexity in auctions have studied how to obtain a near-optimal reserve price based on samples from the distribution $F$ instead of knowing the full distribution.  One of the most important (and most fundamental) price learning algorithms in those works is the \emph{Empirical Revenue Maximization} (ERM) algorithm, which simply outputs the reserve price that is optimal on the uniform distribution over samples (plus some regularization to prevent overfitting). 

\begin{definition}[$c$-Guarded Empirical Revenue Maximization, $\erm^c$]
Draw $N$ samples from a distribution $F$ and sort them non-increasingly, denoted by %$b_1\ge b_2\ge \cdots \ge b_N$.
$v_1\ge v_2\ge \cdots \ge v_N$. 
Given some regularization parameter $0\leq c<1$, choose:
$$ i^* = \argmax_{cN< i \le N}\{i\cdot v_i\},\quad\quad \text{define} ~~ \erm^c(v_1, \ldots, v_N)= v_{i^*}.$$
Assume that the smaller sample (with the larger index) is chosen in case of ties.
\end{definition}

$\erm^c$ was first proposed by~\citet{dhangwatnotai2015revenue} and then extensively studied by~\citet{huang2018making}.  They show that the reserve price output by $\erm^c$ is asymptotically optimal on the underlying distribution $F$ as the number of samples $N$ increases if $F$ is bounded or has monotone hazard rate, with an appropriate choice of $c$.  Other papers have continued to study $\erm^c$, e.g., \cite{babaioff2018two, kanoria2019incentive}. 



%The revenue-optimality of ERM suggests that, in real-world scenarios such as repeated second price auctions, the auctioneer can obtain no-regret revenue by using ERM to update the reserve price at each round of auction based on all previous bids, if buyers are myopic.

However, when ERM is put into practice, it is unclear how the samples can be obtained since many times there is no impartial sampling source.  A natural solution is \emph{endogenous sampling}.
%, by which we mean that the samples are collected from those agents who are part of the auction with reserve price set by ERM.
For example, in repeated second price auctions, the auctioneer can use the bids in previous auctions as samples and run ERM to set a reserve price at each round. But this solution has a challenge of strategic issue: since bidders can affect the determination of future reserve prices, they might have an incentive to underbid in order to increase utility in future auctions.
%But this solution ignores strategic issues since bidders can affect the determination of future reserve prices and therefore might have an incentive to bid strategically in order to increase utility in future auctions.  

Another example of endogenous sampling is the uniform price auction.  In a uniform-price auction the auctioneer sells $N$ copies of a good at some price $p$ to $N$ bidders with i.i.d.~values $\bm{v}$ from $F$ who submit bids $\bm{b}$.  Bidders who bid at least $p$ obtain one copy and pay $p$.  The auctioneer can set the price to be $p=\erm^0(\bm{v})$ to maximize revenue if bids are equal to values.  But \citet{goldberg2006competitive} show that this auction is not incentive-compatible as bidders can lower the price by strategic bidding. 
Therefore, the main question we consider in this paper is:
\begin{center}\emph{To what extent the presence of strategic agents undermines ERM with endogenous sampling?} 
\end{center}
To formally answer the question, we adopt a notion called ``incentive-awareness measure'' originally proposed by \citet{lavi2019redesigning} under bitcoin's fee market context, which measures the reduction of a price learning function $P$ to a change of at most $m$ samples out of the $N$ input samples.

\begin{definition}[Incentive-awareness measures]\label{def:discount}
Let $P:\mathbb{R}_+^N\to\mathbb{R}_+$ be a function (e.g., $\erm^c$) that maps $N$ samples to a reserve price. Draw $N$ i.i.d.~values $v_1, \ldots, v_{N}$ from a distribution $F$. Let $I\subseteq\{1, \ldots, N\}$ be an index set of size $|I|=m$, and $v_I=\{v_i\mid i\in I\}$, $v_{-I}=\{v_j\mid j\notin I\}$. A bidder can change $v_I$ to any $m$ non-negative bids $b_I$, hence change the price from $P(v_I, v_{-I})$ to $P(b_I, v_{-I})$. Define the \emph{incentive-awareness measure}:
$$\delta_I(v_I, v_{-I}) = 1 - \frac{\inf_{b_I\in\mathbb{R}_+^m} P(b_I, v_{-I})}{P(v_I, v_{-I})}, $$
and \emph{worst incentive-awareness measures}: 
\[\delta_{m}^{\interim}(v_{-I}) = \sup_{v_I\in\mathbb{R}_+^m}[ \delta_I(v_I, v_{-I})],\quad\quad\quad\quad\Delta_{N, m}^{\interim} = \E_{v_{-I}\sim F}[ \delta_m^{\interim}(v_{-I})].\]
\end{definition}
A smaller incentive-awareness measure means that the reserve price is decreased by a less amount when a bidder bids strategically.  Since the reduction of reserve price usually increases bidders' utility, a smaller incentive-awareness measure also implies that a bidder cannot benefit a lot from strategic bidding, hence the name ``incentive-awareness measure''.\footnote{\citet{lavi2019redesigning} use the name ``discount ratio'' which we feel can be confused with the standard meaning of a discount ratio in repeated games. % And their definition only consider the case where $m=1$.  The generalization to arbitrary $m\ge 1$ is crucial in our two applications.
}   

\citet{lavi2019redesigning} defined incentive-awareness measures only for $m=1$ and showed that for any distribution $F$ with a finite support size, $\Delta^{\interim}_{N, 1}\to 0$ as $N\to\infty$.  Later, \citet{yao2018incentive} showed that $\Delta^{\interim}_{N, 1}\to 0$ for any continuous distribution with support included in $[1, D]$.  They do not provide specific convergent rates of $\Delta^{\interim}_{N, 1}$.  We generalize their definition to allow $m\ge 1$, which is crucial in our two applications to be discussed.  Our main theoretical contribution is to provide upper bounds on $\Delta^{\interim}_{N, m}$ for two types of value distributions $F$: the class of Monotone Hazard Rate (MHR) distributions where $\frac{f(v)}{1-F(v)}$ is non-decreasing over the support of the distribution (we use $F$ to denote the CDF and $f$ for PDF)
and the class of bounded distributions which consists of all (continuous and discontinuous) distributions with support included in $[1, D]$.  MHR distribution can be unbounded so we are the first to consider incentive-awareness measures for unbounded distributions. 

\begin{theorem}[Main]\label{thm:discount_combined}
Let $P=\erm^c$. The worst incentive-awareness measure is bounded by
\begin{itemize} 
    %\setlength\itemsep{1em}
    \item for MHR $F$, 
    $\Delta^{\interim}_{N, m}=O\left(m\frac{\log^3 N} {\sqrt{N}}\right)$
    , if $m=o(\sqrt{N})$ and $\frac{m}{N}\le c\le\cupperboundmhr$.\footnote{We use $a(n)=o(b(n))$ to denote $\lim_{n\to+\infty}\frac{a(n)}{b(n)}=0$.}
    %\setlength\itemsep{1em}
    \item for bounded $F$, $\Delta^{\interim}_{N, m} = O\left(D^{8/3}m^{2/3}\frac{\log^2 N} {N^{1/3}}\right)$, if $m=o(\sqrt{N})$ and  $\frac{m}{N}\le c\le \frac{1}{2D}$. 
\end{itemize}

The constants in the two big $O$'s are independent of $F$ and $c$. 
\end{theorem}

This theorem implies that as long as the fraction of samples controlled by a bidder is relatively small, the strategic behavior of each bidder has little impact on ERM provided that other bidders are truthful.   

As two applications of our main theorem, we show that (1) a two-phase algorithm that uses $\erm^c$ to update the reserve price in repeated second price auctions can achieve approximate incentive-compatibility and approximate revenue-optimality simultaneously when bidders are non-myopic (Section~\ref{sec:two_phase}); (2) the uniform-auction that sets the price by $\erm^c$ is approximately group incentive-compatible (Section~\ref{sec:uniform-price}).  Finally, we give an overview of the proof of Theorem~\ref{thm:discount_combined} and discuss lower bounds and distributions beyond bounded and MHR distributions in Section~\ref{sec:discussion}. 

% older
%% It is a classic tactic for traditional entrepreneurs to adopt so-called ``personalized (reserve) price" when selling goods to or running auctions for a huge amount of buyers. Intuitively, these buyers can be divided into many groups, according to some statistic information such as how many times they have participated and the total amount of money they have paid, as well as some individual information such as their residents and ages. Buyers in each group share similar features, so that they are believed to have similar value distributions or budgets. For each of these groups, companies are able to analyze their previous transaction data, to determine a specific (reserve) price for more revenue, social welfare, or other objectives.  

%% It has recently become overwhelmingly popular for Internet platform competitions, since deep learning technique is widely used. Basically, deep neural networks are commonly used as classifiers in this circumstance, with participant's features as the input and classification results as the output. Such an end-to-end process plays the same role when dividing buyers into different groups but is usually more efficient and effective.

%% However, these (reserve) prices are not exactly ``personalized", since each group consists of at least thousands of buyers. From the view of efficient implementation, it is still very important how to design anonymous (reserve) price for each group of buyers for specific objectives. \textbf{(what companies are doing)}

% old
% There is currently a trend for Internet companies to adopt so-called ``personalized prices" when selling goods to or running auctions for a large amount of buyers. 
% At a high level, these buyers are partitioned to many groups, according to some common statistical information such as how many times they have participated and the total amount of funds they have paid, as well as some individual information such as their physical locations and age groups. Buyers in each group share similar features, so that they are believed to have similar value distributions. For each of these groups, these Internet companies are able to analyze previous transaction data, to determine a specific reserve price in order to optimize revenue.

% The term ``personalized" is misleading since each such group consists of at least thousands of buyers, and an anonymous reserve price is used on all members in the group for the purpose of computational efficiency. 
% %??? please add reference pointing to the thousands buyers in a group.
% %implementation, it is very important to design anonymous (reserve) price for each group of buyers.
% %and the statistical data of the entire group is used on each of its members in an identical way.
% %In fact, many times, a simple second price auction with an anonymous reserve price is used.
% This practice seems to be supported by auction theory: It is well-known since \citet{myerson1981optimal} that, given that all group members
% have values that are independently and identically drawn from a regular distribution, the revenue-maximizing auction to use is the simple second price auction with an anonymous reserve price. This auction is incentive-compatible, and Myerson specifies an exact formula for the optimal reserve price which requires an exact knowledge of the underlying distribution of values.

% In reality, the exact distribution of values is not known and these Internet companies often treat bids contained in transaction data gathered from each group of buyers as samples from an unknown distribution, in an attempt to infer from it the optimal reserve price to use in Myerson's auction for this group. An interesting theoretical as well as practical question in this context is how %to find the best way
% to determine the optimal reserve price if instead of knowing the exact distribution, the auctioneer has access to $N$ samples from the distribution. A relatively recent literature on sample complexity in auctions has begun to study this algorithmic question. This literature suggests algorithms that compute a reserve price (using these $N$ samples) that leads to a near optimal expected revenue. One of the popular algorithms that was suggested is the Empirical Revenue Maximization (ERM) algorithm. This algorithm was first proposed by~\citet{dhangwatnotai2015revenue} and then extensively studied by~\citet{huang2018making}. They show that the convergence rate of the revenue of ERM to the optimal revenue is in the order of $N^{-\beta}$, where $0<\beta<1$ is characterized for various distribution classes, e.g., MHR distributions or bounded distributions. In other words, ERM is asymptotically optimal for these distributions. Other papers have continued to study ERM such as \citet{babaioff2018two}, who show that the revenue of ERM for any regular distribution and with just two samples is strictly larger than one-half of the optimal revenue, and \citet{kanoria2019incentive}, who use ERM to determine personalized reserve prices in repeated second-price auctions. 

% The theoretical literature on ERM completely ignores the question of how these samples can be obtained. As discussed above, the practical solution used by many Internet companies is to endogenously obtain the samples at first, by initially repeatedly running some truthful auction (for example a second price auction) in order to gather data. Then, after obtaining enough data, use it to compute a suitable reserve price to increase revenue. This solution might be too na\"ive since it ignores strategic issues -- bidders can affect the determination of future reserve prices and therefore might have an incentive to bid strategically in the initial auctions in order to increase utility in future auctions. All previous analyses of ERM completely ignore these two related issues of how would the samples be obtained, and whether the na\"ive solution of endogenously collecting the samples has a significant effect on ERM in the presence of strategic bidders. Other literature has attempted to design more complicated but incentive-compatible sampling techniques. For example, ~\citet{kanoria2019incentive} integrate ERM with (true) personalized pricing in a dynamic way in order to restore incentive-compatibility while obtaining approximate revenue optimality. However, most of these techniques are not used in practice due to various implementability reasons (e.g., computational constraints). On the other hand, in a different (static) context, \citet{azevedo2018strategy} define the notion of ``strategyproofness in the large'' and show that in many natural mechanisms, when there are many bidders, the gain of each bidder from being non-truthful is negligible. One can imagine that a similar phenomenon might hold in our context as well.

% This paper lays out a formal model to analyze the incentive issues created by the na\"ive solution of ERM with endogenous sampling. Using this model, we show that strategyproofness in the large holds here as well, and quantify the relation between the various parameters (number of auctions, length of the sampling period, size of each auction) that suffices in order to simultaneously obtain approximate truthfulness and approximate revenue optimality.
% In this respect, we show that in fact when the market is large the strategic issues are not as problematic as one may imagine initially.

% \paragraph{Model and results.}
% More specifically, we study a model where $T=T_1+T_2$ multiple second price auctions are held in two phases. The first $T_1$ auctions are held with no reserve price, and then $T_2$ auctions use a reserve price calculated by some function $P$ of the bid values (``samples'') from the first phase. Most of our results assume that $P$ is a variant of ERM. Bidders' values in every auction are independently and identically drawn from an (unknown) distribution $F$.\footnote{The other case, when a bidder has a fixed values throughout the two phases, enables the auctioneer to fully infer the second-phase values from the first-phase bids. In such cases, clearly it does not make any sense to perform endogenous sampling. Our attention is therefore focused on the case where the same bidders exhibit newly drawn values in each auction.}
% While bidding in the second phase is incentive-compatible, in the first phase bidders face two contradicting strategic considerations. On the one hand, bidding truthfully in a first-phase auction maximizes a bidder's utility since the auction is incentive-compatible. On the other hand, truthfully disclosing the bidder's true value might increase the resulting reserve price in the second phase, which has a negative effect on the bidder's expected utility in the second phase.
% %Thus, few auctions in the first phase and many auctions in the second phase hurt truthfulness in the first phase as the loss from non-truthful bidding (i.e., losing in the first phase) is small compared to the gain from manipulating the reserve price in the second phase. On the other hand, many auctions in the first phase are problematic as we do not have good revenue guarantees in the first phase.

% Our main result shows that truthful bidding in the first phase is an $\epsilon_1$ Bayes-Nash equilibrium.
% Specifically, letting $N_1$ denote the total number of bids in the first phase, we show that $\epsilon_1 = O(N_1^{-1/2} \log^3 N_1)$ for MHR distributions and  $\epsilon_1 = O(N_1^{-1/3} \log^2 N_1)$ for distributions with a bounded support $[1,D]$, assuming each bidder participates in at most a constant number of auctions. We discuss other distributions in \cref{sec:unbounded-regular-distributions}.\footnote{In particular, we remark in that section that our results can be generalized to the class of $\alpha$-strongly regular distributions~\citet{cole2014the}, with any $\alpha > 0$, and discuss the technical obstacles of generalizing our results to the class of unbounded regular distributions. Note that the class of regular distributions is the largest we can consider since
% running a second price auction with an anonymous reserve price may not be optimal if the distribution is non-regular \citet{myerson1981optimal}.}
% %for revenue optimality,
% Note that $N_1$ increases with both $T_1$ and the number of bidders that participate in the first-phase auctions.
% As these parameters increase, a bidder's benefit from being non-truthful decreases. However, conducting many auctions in the first phase is problematic as we do not have good revenue guarantees in the first phase. The auctioneer therefore needs to carefully balance $T_1$ versus $T_2$. We prove that, assuming truthful bidding, the total expected revenue from the $T$ auctions is at least $(1-\epsilon_2)$ times Myerson's total expected revenue from these $T$ auctions, where $\epsilon_2 = O(T_1/T + \epsilon_1)$. It is therefore possible to set $T_1$ and $T_2$ such that both $\epsilon_1$ and $\epsilon_2$ will go to zero as $T\rightarrow \infty$.
% %
% Our results are in fact more general and incorporate additional parameters, mainly an upper bound $\msum$ on the number of auctions that each bidder participates in. For simplicity, the above statements assume that this parameter is constant, but our actual results allow non-constant $\msum=o(\sqrt{N_1})$ (Theorem~\ref{thm:TPM_utility_revenue_combined}). 


% %technical overview
% %incentive-awareness measure, delta interim, the connection to the above, application to uniform-price auctions
% \paragraph{Techniques.}
% Our technical analysis relies on an ``incentive-awareness measure'' notion that measures the amount of influence that a bidder can have on the price learning function $P$. Let
% $I$ be a subset of indices from $\{1, \ldots, N\}$. For some vector of bidder values $(v_I, v_{-I})$, a bidder that provides a subset $v_I$ of the samples can try to manipulate and provide false samples $b^*_I$ to decrease the reserve price to $\inf_{b_I\in\mathbb{R}_+^m} P(b_I, v_{-I})$. The incentive-awareness measure
% $\delta_I(v_I, v_{-I}) \coloneqq 1 - P(b^*_I, v_{-I})/P(v_I, v_{-I})$ measures the amount of influence one can have by changing $m=|I|$ samples. Let $\Delta_{N, m}^{\interim}$ be the expected value of the incentive-awareness measure. This notion is useful for the analysis of the two-phase model since we prove that $\epsilon_1 = O(\Delta^{\interim}_{N=N_1, \msum})$. As another application, we mention in the paper a connection to the classic model of uniform price auctions. The main technical challenge is to characterize the rate of convergence of $\Delta_{N, m}^{\interim}$ to zero as $N \rightarrow \infty$, for MHR and for bounded distributions, when $P=\erm$ (Theorem~\ref{thm:discount_combined}). 



% \paragraph{Structure of the paper.} Some additional related literature is discussed in section \ref{sec:related_work}. The model and additional notation and other technical preliminaries are given in Section \ref{sec:preliminaries}.
% Section~\ref{sec:discount-ratio-definition} formally defines the notion of an incentive-awareness measure and gives an overview of the main results regarding this technical tool. Section~\ref{sec:two_phase} then gives as corollaries our main results regarding the two-phase model plus additional two extensions, to the case of multiple units (more than a single item in each auction) and to the case of multiple periods (more than two periods). Section~\ref{sec:discount_ratio_upper-bound} gives a detailed technical overview of the proof of the upper bound on the incentive-awareness measure, with missing details given in the appendix. Section~\ref{sec:discussion} discusses some additional issues, including an application of our analysis of the incentive-awareness measure to the classic model of uniform-price auctions, lower bounds on the incentive-awareness measure and our two-phase model, and a discussion on unbounded regular distributions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Related Works}
\label{sec:related_work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Sample complexity in auctions.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Previous works on ERM mainly focus on its sample complexity, started by \citet{cole2014the}. While ERM is suitable for the case of i.i.d.~values (e.g., \cite{huang2018making}), the literature on sample complexity has expanded to more general cases of independent but non-identical values and multi-dimensional values, e.g.~\cite{morgenstern2015pseudo, devanur2016sample, gonczarowski2018sample, guo2019settling}, or replacing second price auction by a restricted family of non-truthful auctions, e.g.~\cite{hartline2018sample}.  \citet{babaioff2018two} study the performance of ERM with just two samples. 
%, and \citet{kanoria2019incentive} determining personalized reserve prices in repeated second-price auctions by ERM.  %which is generalized to contextual setting by \citet{NIPS2019_Golrezaei_dynamic}.
While this literature assumes that samples are exogenous, our main contribution is to consider endogenous samples that are collected from bidders who will be affected by the outcome of the learning algorithm. 
%participates in later auctions as well.


% One of the first papers to study the issue of sample complexity for revenue maximization is~\citet{cole2014the}. While $\erm$ is suitable for the case of i.i.d.~values (e.g., \citet{huang2018making}), the literature on sample complexity has expanded to more general cases of independent but non-identical values and multi-dimensional values, see e.g.,~\citet{morgenstern2015pseudo, devanur2016sample, gonczarowski2018sample, guo2019settling}. While all these papers study truthful auctions, \citet{hartline2018sample} show that a polynomial number of samples from the bid distribution are sufficient to identify an auction within a restricted family of non-truthful auctions that approximates the overall optimal auction.
% While this literature assumes that samples are exogenous, our main contribution is to consider endogenous samples that are collected from the same set of bidders that participates in later auctions as well.


%%\paragraph{Reserve price learning without incentive-awareness.}
%%There are some works \citet{cesa2015regret, medina2014learning} about learning an optimal reserve price in second price auctions. For example,  \citet{cesa2015regret} studies the problem of learning reserve prices in repeated second price auctions in a no-regret manner.
%%\citet{medina2014learning} studies the problem from a theoretical perspective.
%The major deficiency of this line of works is the ignorance of incentive issues, because they assume that the bids are drawn from a fixed distribution which does not depend on the reserve price learning algorithm. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Incentive-aware learning.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Repeated auctions against non-myopic bidders.}
Besides ERM, early papers consider tools from learning theory to approximately maximize revenue without knowing exact distributions, for example, in the static (one shot) setting \cite{balcan2008reducing}, in online setting with myopic bidders \cite{blum2005near, medina2014learning, cesa2015regret, bubeck2017online}, and with non-myopic strategic bidders~\cite{amin2013learning, amin2014repeated,NIPS2019_deng_robust,NIPS2019_Golrezaei_dynamic}.
\citet{epasto2018incentive} also consider randomly choosing reserve price to maintain approximate truthfulness and revenue when there is no underlying distribution.
Our study on the incentive issue in the endogenous sampling is more related to \cite{liu2018learning} and \cite{NIPS2019_abernethy_learning}, who adopt differential privacy technique to bound bidders' manipulation on samples. Comparing with them, our ERM is more practical as it is much simpler, and their algorithms rely on the boundedness of value distributions while we allow unbounded distributions. Furthermore, their results require a large number of auctions while ours need a large number of samples which can be obtained by either few bids in many auctions, many bids in few auctions, or combined.


% Early papers describe how to employ tools from learning theory in order to approximately maximize revenue in the static (one shot) setting, for example \citet{balcan2008reducing}. In the online case, no-regret online learning has been proposed as a way to learn the optimal reserve price, both for myopic bidders~\citet{blum2005near, medina2014learning, cesa2015regret, bubeck2017online} as well as for non-myopic strategic bidders~\citet{amin2013learning, amin2014repeated,NIPS2019_deng_robust,NIPS2019_Golrezaei_dynamic}. More recently,~\citet{liu2018learning} and \citet{NIPS2019_abernethy_learning} address the technical challenge of designing the online learning algorithm in an (approximately) incentive compatible way, since bidders may participate in more than one round of the online process. Three main differences between this literature and our model are: (1) they use differentially private algorithms to design approximately truthful repeated auctions while we use ERM which seems more practical due to its simplicity compared to complicated pricing solutions using, e.g., differential privacy;
% (2) their algorithms inevitably rely on the boundedness of value distributions while we allow unbounded distributions; (3) they need a large number of auctions while we need a large number of samples which can be obtained by either few bids in many auctions, many bids in few auctions, or combined.
% %We also believe that ERM is more applicable to practice due to its simplicity compared to complicated pricing solutions using, e.g., differential privacy.
% \citet{epasto2018incentive} show how to randomly choose a reserve price in a way that depends on bidders' bids and still maintains (1) approximate truthfulness and (2) revenue which is close to the optimal revenue obtained with any reserve price. It characterizes the trade-off between these two properties by a parameter which they term the ``learning rate''. In contrast to our model, there is no underlying distribution and hence no attempt to learn the optimal reserve price for the underlying distribution.
% Other literature has attempted to design more complicated but incentive-compatible sampling techniques. For example, ~\citet{kanoria2019incentive} integrate ERM with (true) personalized pricing in a dynamic way in order to restore incentive-compatibility while obtaining approximate revenue optimality. However, most of these techniques are not used in practice due to various implementability reasons (e.g., computational constraints). On the other hand, in a different (static) context, \citet{azevedo2018strategy} define the notion of ``strategyproofness in the large'' and show that in many natural mechanisms, when there are many bidders, the gain of each bidder from being non-truthful is negligible. One can imagine that a similar phenomenon might hold in our context as well.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Equilibrium analysis.}
% \new{shorten this, move to appendix, or move to repeated auctions against non-myopic bidders}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A few papers have analyzed equilibria in a setting with $T$ rounds and $n$ bidders that participate in each round, where the auctioneer is updating the reserve price based on past bids. For example,~\citet{kanoria2019incentive} prove that it is not possible to set a common reserve price that depends on previous bids in a way that maintains truthfulness. It then suggests a method by setting personalized reserve prices using $\erm$ which is clearly truthful and obtains revenue that approaches the optimal revenue as $T$ goes to infinity. A follow-up paper by~\citet{NIPS2019_Golrezaei_dynamic}
% %\item Dynamic Incentive-aware Learning: Robust Pricing in Contextual Auctions
% generalizes the model to the case of correlated values and studies other algorithms (instead of $\erm$) to be used as the personalized pricing algorithms. In contrast to these two papers, we focus on the case of a common reserve price, quantifying exactly how the incentive to deviate from truthfulness decreases as the number of bidders increases.
% When values are drawn at the beginning of the game from some regular distribution and stay fixed throughout, \citet{immorlica2017repeated} show that, while with a single buyer the equilibrium revenue is far from optimal, with two or more buyers there exists a perfect Bayesian equilibrium in which the revenue is a constant fraction of the optimal revenue.

\paragraph{Equilibrium analysis.}
Instead of auction design, a few papers also do equilibrium analysis for common repeat auction mechanisms, for example \cite{kanoria2019incentive} and \cite{NIPS2019_Golrezaei_dynamic}. Precisely, the corresponding dynamic game is an auction with $T$ rounds and $n$ bidders that participate in each round, where the auctioneer is updating the reserve price based on past bids.
The equilibrium results in \cite{immorlica2017repeated} are similar to us, as they show with fixed value from some regular distribution, the equilibrium revenue for a single buyer is far from optimal, while there exists a perfect Bayesian equilibrium in which the revenue is a constant fraction of the optimal revenue for two or more buyers.
In comparison, we focus on quantifying exactly how the incentive to deviate from truthfulness decreases as the number of bidders increases.
%In this respect, both results can be regarded as a similar phenomenon called ``strategyproofness in the large'', defined by \citet{azevedo2018strategy} who show that in many natural mechanisms, when there are many bidders, the gain of each bidder from being non-truthful is negligible. 

==> ec_abstract.tex <==
% short
We study the endogenous incentiveness in learning algorithms for revenue-maximizing auctions.
The recent literature on sample-complexity in auctions studies a setting where the auctioneer does not know the underlying value distribution and instead has access to several samples from it. This literature does not consider the source of these samples.
In particular, in reality, the fact that samples are collected from bidders who also participate in future auctions creates an incentive for these bidders to misreport true values in the sampling process.
We formalize this problem as a two-phase game where in the first phase an auctioneer runs multiple second-price auctions, and in the second phase it uses the Empirical Revenue Maximization algorithm to determine a reserve price in all second-phase auctions that will induce an approximately optimal revenue, based on the bids observed in the first phase.
We show that truthful bidding is an $\epsilon_1$-BNE in this setting, and by further appropriately choosing the number of auctions in the two phases, we can also obtain $(1-\epsilon_2)$ approximate revenue optimality, where $\epsilon_1$ and $\epsilon_2$ go to zero as the number of bids and the number of auctions go to infinity.
The proof of our main result relies on an analysis of an ``incentive-awareness measure'' of a reserve price learning function, which we believe is of independent interest.





% old
% The recent literature on sample-complexity in auctions studies a setting where the auctioneer does not know the underlying value distribution and instead has access to several samples from it. This literature does not consider the source of these samples.
% In particular, in reality, the fact that samples are collected from bidders who also participate in future auctions creates an incentive for these bidders to misreport true values in the sampling process.
% %
% We study a two-phase model where in the first phase an auctioneer runs multiple second-price auctions (or any other auction which is truthful in the standard static setting), and in the second phase it uses the Empirical Revenue Maximization algorithm to determine a reserve price in all second-phase auctions that will induce an approximately optimal revenue, based on the bids observed in the first phase. Bidders' values in each auction are i.i.d.~from an arbitrary bounded or MHR distribution which is unknown to the auctioneer. Our main result shows that truthfulness is an $\epsilon_1$-BNE in this setting, where $\epsilon_1$ goes to zero as the total number of bids in the first-phase auctions, $N$, goes to infinity.
% Specifically, $\epsilon_1 = O(N^{-1/3}\log^2 N)$ for bounded distributions and $\epsilon_1 = O(N^{-1/2}\log^3 N)$ for MHR distributions. 
% %at a rate which is not slower than $O(N^{-1/3}\log^2 N)$.
% We also show that, by appropriately choosing the number of auctions in the two phases, we simultaneously obtain $(1-\epsilon_2)$ approximate revenue optimality together with approximate truthfulness where $\epsilon_2$ also goes to zero as the number of bids and the number of auctions go to infinity. The proof of our main result relies on an analysis of an ``incentive-awareness measure'' of a reserve price learning function, which we believe is of independent interest.

==> old_intro+model.tex <==
% \new{we need to shorten the intro, and justify iid setting and the study of ERM}

In auction theory, it is well-known since \citet{myerson1981optimal} that, given that all buyers have values that are independently and identically drawn from a regular distribution, the revenue-maximizing auction to use is the simple second price auction with an anonymous reserve price. 
This theory is well applied by Internet companies when selling goods to or running auctions for a large amount of buyers. 
At a high level, these buyers are partitioned to many groups, where buyers in each group, sharing similar statistical features or individual properties, are believed to have similar value distributions. For each of these groups, these Internet companies are able to analyze previous transaction data, determine a specific reserve price, run corresponding auctions in order to optimize revenue.
% At a high level, these buyers are partitioned to many groups, according to some common statistical information such as how many times they have participated and the total amount of funds they have paid, as well as some individual information such as their physical locations and age groups. Buyers in each group share similar features, so that they are believed to have similar value distributions. For each of these groups, these Internet companies are able to analyze previous transaction data, to determine a specific reserve price in order to optimize revenue.
% Although such a group division is often referred to as adopting ``personalized prices", the term ``personalized" is misleading since each such group consists of at least thousands of buyers, and an anonymous reserve price is used on all members in the group for the purpose of computational efficiency. 

Myerson's formula for the optimal reserve price %and proof for its incentive-compatibility 
relies on an exact knowledge of the underlying distribution of values.
However, in reality, the Internet companies do not know the value distribution of buyers, but have access to samples of their bids in previous transactions. 
To determine the optimal reserve price based on these samples without knowing the exact distribution, one of the most popular algorithms is the Empirical Revenue Maximization (ERM) algorithm, which computes a reserve price that is optimal on the uniform distribution over samples. %that leads to a near optimal expected revenue.
ERM was first proposed by~\citet{dhangwatnotai2015revenue} and then extensively studied by~\citet{huang2018making}. They show that the reserve price outputted by ERM is asymptotically optimal on the underlying distribution as the number of samples $N$ increases if the underlying distribution is bounded or has monotone hazard rate (MHR). 
%belongs to MHR distributions or bounded distributions. 

However, previous theoretical literature on ERM completely ignores the question of how these samples can be obtained. Precisely, the data samples used to compute a reserve price are usually gathered by repeatedly running some truthful auction (for example a second price auction). When these bidders realize that they can influence the reserve prices of the auctions they will participant in the future, they might have an incentive to bid strategically in these initial auctions in order to increase their total utilities.
Thus, a nature challenge for applying ERM is the problem that whether the na\"ive solution of endogenously collecting the samples has a significant effect on ERM in the presence of strategic bidders. 

To quantify the incentive issues created by the ERM algorithm with endogenous sampling, we introduce an incentive-awareness measure, generalized from the definition proposed by \citet{lavi2019redesigning} and \citet{yao2018incentive}, to upper bound the reduction of ERM's outputted price due to any change of $m\ge 1$ out of $N$ input samples. We provide the specific convergence rates of this measure to zero as $N$ goes to infinity for both bounded distributions and MHR distributions, showing that ERM is relatively robust against bidders' strategic manipulation on their bidding samples. 
Moreover, we use the ERM algorithm to design repeated auctions and uniform-price auctions as its applications, whose revenue-optimility and truthfulness against non-myopic bidders can be guaranteed by ERM's asymptotically convergent incentive-awareness measure.



% older
%% It is a classic tactic for traditional entrepreneurs to adopt so-called ``personalized (reserve) price" when selling goods to or running auctions for a huge amount of buyers. Intuitively, these buyers can be divided into many groups, according to some statistic information such as how many times they have participated and the total amount of money they have paid, as well as some individual information such as their residents and ages. Buyers in each group share similar features, so that they are believed to have similar value distributions or budgets. For each of these groups, companies are able to analyze their previous transaction data, to determine a specific (reserve) price for more revenue, social welfare, or other objectives.  

%% It has recently become overwhelmingly popular for Internet platform competitions, since deep learning technique is widely used. Basically, deep neural networks are commonly used as classifiers in this circumstance, with participant's features as the input and classification results as the output. Such an end-to-end process plays the same role when dividing buyers into different groups but is usually more efficient and effective.

%% However, these (reserve) prices are not exactly ``personalized", since each group consists of at least thousands of buyers. From the view of efficient implementation, it is still very important how to design anonymous (reserve) price for each group of buyers for specific objectives. \textbf{(what companies are doing)}

% old
% There is currently a trend for Internet companies to adopt so-called ``personalized prices" when selling goods to or running auctions for a large amount of buyers. 
% At a high level, these buyers are partitioned to many groups, according to some common statistical information such as how many times they have participated and the total amount of funds they have paid, as well as some individual information such as their physical locations and age groups. Buyers in each group share similar features, so that they are believed to have similar value distributions. For each of these groups, these Internet companies are able to analyze previous transaction data, to determine a specific reserve price in order to optimize revenue.

% The term ``personalized" is misleading since each such group consists of at least thousands of buyers, and an anonymous reserve price is used on all members in the group for the purpose of computational efficiency. 
% %??? please add reference pointing to the thousands buyers in a group.
% %implementation, it is very important to design anonymous (reserve) price for each group of buyers.
% %and the statistical data of the entire group is used on each of its members in an identical way.
% %In fact, many times, a simple second price auction with an anonymous reserve price is used.
% This practice seems to be supported by auction theory: It is well-known since \citet{myerson1981optimal} that, given that all group members
% have values that are independently and identically drawn from a regular distribution, the revenue-maximizing auction to use is the simple second price auction with an anonymous reserve price. This auction is incentive-compatible, and Myerson specifies an exact formula for the optimal reserve price which requires an exact knowledge of the underlying distribution of values.

% In reality, the exact distribution of values is not known and these Internet companies often treat bids contained in transaction data gathered from each group of buyers as samples from an unknown distribution, in an attempt to infer from it the optimal reserve price to use in Myerson's auction for this group. An interesting theoretical as well as practical question in this context is how %to find the best way
% to determine the optimal reserve price if instead of knowing the exact distribution, the auctioneer has access to $N$ samples from the distribution. A relatively recent literature on sample complexity in auctions has begun to study this algorithmic question. This literature suggests algorithms that compute a reserve price (using these $N$ samples) that leads to a near optimal expected revenue. One of the popular algorithms that was suggested is the Empirical Revenue Maximization (ERM) algorithm. This algorithm was first proposed by~\citet{dhangwatnotai2015revenue} and then extensively studied by~\citet{huang2018making}. They show that the convergence rate of the revenue of ERM to the optimal revenue is in the order of $N^{-\beta}$, where $0<\beta<1$ is characterized for various distribution classes, e.g., MHR distributions or bounded distributions. In other words, ERM is asymptotically optimal for these distributions. Other papers have continued to study ERM such as \citet{babaioff2018two}, who show that the revenue of ERM for any regular distribution and with just two samples is strictly larger than one-half of the optimal revenue, and \citet{kanoria2019incentive}, who use ERM to determine personalized reserve prices in repeated second-price auctions. 

% The theoretical literature on ERM completely ignores the question of how these samples can be obtained. As discussed above, the practical solution used by many Internet companies is to endogenously obtain the samples at first, by initially repeatedly running some truthful auction (for example a second price auction) in order to gather data. Then, after obtaining enough data, use it to compute a suitable reserve price to increase revenue. This solution might be too na\"ive since it ignores strategic issues -- bidders can affect the determination of future reserve prices and therefore might have an incentive to bid strategically in the initial auctions in order to increase utility in future auctions. All previous analyses of ERM completely ignore these two related issues of how would the samples be obtained, and whether the na\"ive solution of endogenously collecting the samples has a significant effect on ERM in the presence of strategic bidders. Other literature has attempted to design more complicated but incentive-compatible sampling techniques. For example, ~\citet{kanoria2019incentive} integrate ERM with (true) personalized pricing in a dynamic way in order to restore incentive-compatibility while obtaining approximate revenue optimality. However, most of these techniques are not used in practice due to various implementability reasons (e.g., computational constraints). On the other hand, in a different (static) context, \citet{azevedo2018strategy} define the notion of ``strategyproofness in the large'' and show that in many natural mechanisms, when there are many bidders, the gain of each bidder from being non-truthful is negligible. One can imagine that a similar phenomenon might hold in our context as well.

% This paper lays out a formal model to analyze the incentive issues created by the na\"ive solution of ERM with endogenous sampling. Using this model, we show that strategyproofness in the large holds here as well, and quantify the relation between the various parameters (number of auctions, length of the sampling period, size of each auction) that suffices in order to simultaneously obtain approximate truthfulness and approximate revenue optimality.
% In this respect, we show that in fact when the market is large the strategic issues are not as problematic as one may imagine initially.

% \paragraph{Model and results.}
% More specifically, we study a model where $T=T_1+T_2$ multiple second price auctions are held in two phases. The first $T_1$ auctions are held with no reserve price, and then $T_2$ auctions use a reserve price calculated by some function $P$ of the bid values (``samples'') from the first phase. Most of our results assume that $P$ is a variant of ERM. Bidders' values in every auction are independently and identically drawn from an (unknown) distribution $F$.\footnote{The other case, when a bidder has a fixed values throughout the two phases, enables the auctioneer to fully infer the second-phase values from the first-phase bids. In such cases, clearly it does not make any sense to perform endogenous sampling. Our attention is therefore focused on the case where the same bidders exhibit newly drawn values in each auction.}
% While bidding in the second phase is incentive-compatible, in the first phase bidders face two contradicting strategic considerations. On the one hand, bidding truthfully in a first-phase auction maximizes a bidder's utility since the auction is incentive-compatible. On the other hand, truthfully disclosing the bidder's true value might increase the resulting reserve price in the second phase, which has a negative effect on the bidder's expected utility in the second phase.
% %Thus, few auctions in the first phase and many auctions in the second phase hurt truthfulness in the first phase as the loss from non-truthful bidding (i.e., losing in the first phase) is small compared to the gain from manipulating the reserve price in the second phase. On the other hand, many auctions in the first phase are problematic as we do not have good revenue guarantees in the first phase.

% Our main result shows that truthful bidding in the first phase is an $\epsilon_1$ Bayes-Nash equilibrium.
% Specifically, letting $N_1$ denote the total number of bids in the first phase, we show that $\epsilon_1 = O(N_1^{-1/2} \log^3 N_1)$ for MHR distributions and  $\epsilon_1 = O(N_1^{-1/3} \log^2 N_1)$ for distributions with a bounded support $[1,D]$, assuming each bidder participates in at most a constant number of auctions. We discuss other distributions in \cref{sec:unbounded-regular-distributions}.\footnote{In particular, we remark in that section that our results can be generalized to the class of $\alpha$-strongly regular distributions~\citet{cole2014the}, with any $\alpha > 0$, and discuss the technical obstacles of generalizing our results to the class of unbounded regular distributions. Note that the class of regular distributions is the largest we can consider since
% running a second price auction with an anonymous reserve price may not be optimal if the distribution is non-regular \citet{myerson1981optimal}.}
% %for revenue optimality,
% Note that $N_1$ increases with both $T_1$ and the number of bidders that participate in the first-phase auctions.
% As these parameters increase, a bidder's benefit from being non-truthful decreases. However, conducting many auctions in the first phase is problematic as we do not have good revenue guarantees in the first phase. The auctioneer therefore needs to carefully balance $T_1$ versus $T_2$. We prove that, assuming truthful bidding, the total expected revenue from the $T$ auctions is at least $(1-\epsilon_2)$ times Myerson's total expected revenue from these $T$ auctions, where $\epsilon_2 = O(T_1/T + \epsilon_1)$. It is therefore possible to set $T_1$ and $T_2$ such that both $\epsilon_1$ and $\epsilon_2$ will go to zero as $T\rightarrow \infty$.
% %
% Our results are in fact more general and incorporate additional parameters, mainly an upper bound $\msum$ on the number of auctions that each bidder participates in. For simplicity, the above statements assume that this parameter is constant, but our actual results allow non-constant $\msum=o(\sqrt{N_1})$ (Theorem~\ref{thm:TPM_utility_revenue_combined}). 


% %technical overview
% %incentive-awareness measure, delta interim, the connection to the above, application to uniform-price auctions
% \paragraph{Techniques.}
% Our technical analysis relies on an ``incentive-awareness measure'' notion that measures the amount of influence that a bidder can have on the price learning function $P$. Let
% $I$ be a subset of indices from $\{1, \ldots, N\}$. For some vector of bidder values $(v_I, v_{-I})$, a bidder that provides a subset $v_I$ of the samples can try to manipulate and provide false samples $b^*_I$ to decrease the reserve price to $\inf_{b_I\in\mathbb{R}_+^m} P(b_I, v_{-I})$. The incentive-awareness measure
% $\delta_I(v_I, v_{-I}) \coloneqq 1 - P(b^*_I, v_{-I})/P(v_I, v_{-I})$ measures the amount of influence one can have by changing $m=|I|$ samples. Let $\Delta_{N, m}^{\interim}$ be the expected value of the incentive-awareness measure. This notion is useful for the analysis of the two-phase model since we prove that $\epsilon_1 = O(\Delta^{\interim}_{N=N_1, \msum})$. As another application, we mention in the paper a connection to the classic model of uniform price auctions. The main technical challenge is to characterize the rate of convergence of $\Delta_{N, m}^{\interim}$ to zero as $N \rightarrow \infty$, for MHR and for bounded distributions, when $P=\erm$ (Theorem~\ref{thm:discount_combined}). 



% \paragraph{Structure of the paper.} Some additional related literature is discussed in section \ref{sec:related_work}. The model and additional notation and other technical preliminaries are given in Section \ref{sec:preliminaries}.
% Section~\ref{sec:discount-ratio-definition} formally defines the notion of an incentive-awareness measure and gives an overview of the main results regarding this technical tool. Section~\ref{sec:two_phase} then gives as corollaries our main results regarding the two-phase model plus additional two extensions, to the case of multiple units (more than a single item in each auction) and to the case of multiple periods (more than two periods). Section~\ref{sec:discount_ratio_upper-bound} gives a detailed technical overview of the proof of the upper bound on the incentive-awareness measure, with missing details given in the appendix. Section~\ref{sec:discussion} discusses some additional issues, including an application of our analysis of the incentive-awareness measure to the classic model of uniform-price auctions, lower bounds on the incentive-awareness measure and our two-phase model, and a discussion on unbounded regular distributions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Additional Related Literature}
\label{sec:related_work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Sample complexity in auctions.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Previous study on ERM mainly focus on its sample complexity, started by \citet{cole2014the}. While $\erm$ is suitable for the case of i.i.d.~values (e.g., \citet{huang2018making}), the literature on sample complexity has expanded to more general cases of independent but non-identical values and multi-dimensional values, see e.g.,~\citet{morgenstern2015pseudo, devanur2016sample, gonczarowski2018sample, guo2019settling}, or replacing second price auction by a restricted family of non-truthful auctions \citet{hartline2018sample}. Other study on ERM includes computing its revenue with just two samples \cite{babaioff2018two}, and determining personalized reserve prices in repeated second-price auctions by ERM \cite{kanoria2019incentive}.
While this literature assumes that samples are exogenous, our main contribution is to consider endogenous samples that are collected from the same set of bidders that participates in later auctions as well.


% One of the first papers to study the issue of sample complexity for revenue maximization is~\citet{cole2014the}. While $\erm$ is suitable for the case of i.i.d.~values (e.g., \citet{huang2018making}), the literature on sample complexity has expanded to more general cases of independent but non-identical values and multi-dimensional values, see e.g.,~\citet{morgenstern2015pseudo, devanur2016sample, gonczarowski2018sample, guo2019settling}. While all these papers study truthful auctions, \citet{hartline2018sample} show that a polynomial number of samples from the bid distribution are sufficient to identify an auction within a restricted family of non-truthful auctions that approximates the overall optimal auction.
% While this literature assumes that samples are exogenous, our main contribution is to consider endogenous samples that are collected from the same set of bidders that participates in later auctions as well.


%%\paragraph{Reserve price learning without incentive-awareness.}
%%There are some works \citet{cesa2015regret, medina2014learning} about learning an optimal reserve price in second price auctions. For example,  \citet{cesa2015regret} studies the problem of learning reserve prices in repeated second price auctions in a no-regret manner.
%%\citet{medina2014learning} studies the problem from a theoretical perspective.
%The major deficiency of this line of works is the ignorance of incentive issues, because they assume that the bids are drawn from a fixed distribution which does not depend on the reserve price learning algorithm. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \paragraph{Incentive-aware learning.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Besides ERM, early papers consider tools from learning theory to approximately maximize revenue without knowing exact distributions, for example, in the static (one shot) setting \citet{balcan2008reducing}, in online setting with myopic bidders \citet{blum2005near, medina2014learning, cesa2015regret, bubeck2017online}, and with non-myopic strategic bidders~\citet{amin2013learning, amin2014repeated,NIPS2019_deng_robust,NIPS2019_Golrezaei_dynamic}.
\citet{epasto2018incentive} also consider randomly choosing reserve price to maintain approximate truthfulness and revenue when there is no underlying distribution.
Our study on the incentive issue in the endogenous sampling is more related to \citet{liu2018learning} and \citet{NIPS2019_abernethy_learning}, who adopt differential privacy technique to bound bidders' manipulation on samples. Comparing with them, our ERM is more practical as it is much simpler, and their algorithms rely on the boundedness of value distributions while we allow unbounded distributions. Furthermore, their results requires a large number of auctions while ours need a large number of samples which can be obtained by either few bids in many auctions, many bids in few auctions, or combined.
In this respect, both results can be regarded as a similar phenomenon called ``strategyproofness in the large'', defined by \citet{azevedo2018strategy} who show that in many natural mechanisms, when there are many bidders, the gain of each bidder from being non-truthful is negligible. 

% Early papers describe how to employ tools from learning theory in order to approximately maximize revenue in the static (one shot) setting, for example \citet{balcan2008reducing}. In the online case, no-regret online learning has been proposed as a way to learn the optimal reserve price, both for myopic bidders~\citet{blum2005near, medina2014learning, cesa2015regret, bubeck2017online} as well as for non-myopic strategic bidders~\citet{amin2013learning, amin2014repeated,NIPS2019_deng_robust,NIPS2019_Golrezaei_dynamic}. More recently,~\citet{liu2018learning} and \citet{NIPS2019_abernethy_learning} address the technical challenge of designing the online learning algorithm in an (approximately) incentive compatible way, since bidders may participate in more than one round of the online process. Three main differences between this literature and our model are: (1) they use differentially private algorithms to design approximately truthful repeated auctions while we use ERM which seems more practical due to its simplicity compared to complicated pricing solutions using, e.g., differential privacy;
% (2) their algorithms inevitably rely on the boundedness of value distributions while we allow unbounded distributions; (3) they need a large number of auctions while we need a large number of samples which can be obtained by either few bids in many auctions, many bids in few auctions, or combined.
% %We also believe that ERM is more applicable to practice due to its simplicity compared to complicated pricing solutions using, e.g., differential privacy.
% \citet{epasto2018incentive} show how to randomly choose a reserve price in a way that depends on bidders' bids and still maintains (1) approximate truthfulness and (2) revenue which is close to the optimal revenue obtained with any reserve price. It characterizes the trade-off between these two properties by a parameter which they term the ``learning rate''. In contrast to our model, there is no underlying distribution and hence no attempt to learn the optimal reserve price for the underlying distribution.
% Other literature has attempted to design more complicated but incentive-compatible sampling techniques. For example, ~\citet{kanoria2019incentive} integrate ERM with (true) personalized pricing in a dynamic way in order to restore incentive-compatibility while obtaining approximate revenue optimality. However, most of these techniques are not used in practice due to various implementability reasons (e.g., computational constraints). On the other hand, in a different (static) context, \citet{azevedo2018strategy} define the notion of ``strategyproofness in the large'' and show that in many natural mechanisms, when there are many bidders, the gain of each bidder from being non-truthful is negligible. One can imagine that a similar phenomenon might hold in our context as well.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Equilibrium analysis.}
\new{shorten this or move to appendix}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
A few papers have analyzed equilibria in a setting with $T$ rounds and $n$ bidders that participate in each round, where the auctioneer is updating the reserve price based on past bids. For example,~\citet{kanoria2019incentive} prove that it is not possible to set a common reserve price that depends on previous bids in a way that maintains truthfulness. It then suggests a method by setting personalized reserve prices using $\erm$ which is clearly truthful and obtains revenue that approaches the optimal revenue as $T$ goes to infinity. A follow-up paper by~\citet{NIPS2019_Golrezaei_dynamic}
%\item Dynamic Incentive-aware Learning: Robust Pricing in Contextual Auctions
generalizes the model to the case of correlated values and studies other algorithms (instead of $\erm$) to be used as the personalized pricing algorithms. In contrast to these two papers, we focus on the case of a common reserve price, quantifying exactly how the incentive to deviate from truthfulness decreases as the number of bidders increases.
When values are drawn at the beginning of the game from some regular distribution and stay fixed throughout, \citet{immorlica2017repeated} show that, while with a single buyer the equilibrium revenue is far from optimal, with two or more buyers there exists a perfect Bayesian equilibrium in which the revenue is a constant fraction of the optimal revenue.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\paragraph{Revenue-maximization with imprecise distribution (if we include revenue analysis)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\section{Model and Main Results}
\section{Incentive-Aware Price Learning by ERM}
\label{sec:preliminaries}

\new{Should we add some preliminaries on auctions? For example, ``what is second price auction with reserve?''; and ``the optimal reserve is $\argmax\{p[1-F(p)]\}$''. }

\noindent
{\bf Reserve price learning function. }
There are $n$ bidders whose values are independently and identically drawn from a cumulative distribution $F$ which is unknown to the auctioneer. 
There are $N$ samples of these bidders' previous bids for their value, among which each bidder controls at most $m$ bids.
With these samples, a \emph{reserve price learning function}, $P:\mathbb{R}_+^{N} \to \mathbb{R}_+$ is used to determine the reserve price of second price auctions for these bidders.

\noindent
{\bf Empirical Revenue Maximization. }
We focus on the following reserve price learning function $P=\erm^c$.\footnote{\citet{dhangwatnotai2015revenue} and \citet{huang2018making} observe that for some classes of distributions, e.g., MHR distributions, w.h.p.~$\erm$ (the version with $c=0$) and $\erm^c$ will result in the same reserve price when $c \leq \frac{1}{e}$, while for other classes of distributions, $\erm$ does not guarantee approximately optimal revenue and in these cases they have suggested $\erm^c$.}
Suppose the $N$ samples that are sorted non-increasingly, denoted by $b_1\ge b_2\ge \cdots \ge b_N$. 
Given some parameter $0<c<1$, choose:
$$ i^* = \argmax_{cN< i \le N}\{i\cdot b_i\},\quad \quad \erm^c(b_1, \ldots, b_N)\defeq b_{i^*}.$$
Assume that the smaller sample (with the larger index) is chosen in case of ties.

\noindent
{\bf Incentive-awareness measures. }
As each bidder knows the reserve price learning function, he has the incentive to strategically manipulate the samples controlled by him, and further the reserve price, in order to obtain better utility.
The corresponding strategic analysis of a reserve price learning function is closely related to a notion of an ``incentive-awareness measure'' recently studied by~\citet{lavi2019redesigning} and~\citet{yao2018incentive} in a different context, as described next.\footnote{These two papers use the term ``discount ratio'' which we feel can be confused with the standard meaning of a discount ratio in repeated games.}

\begin{definition}[Incentive-awareness measures]\label{def:discount}
Draw $N$ i.i.d.~values $v_1, \ldots, v_{N}$ from a distribution $F$. Let $I\subseteq\{1, \ldots, N\}$ be an index set of size $|I|=m$, and $v_I=\{v_i\mid i\in I\}$, $v_{-I}=\{v_j\mid j\notin I\}$. A bidder can change $v_I$ to any $m$ non-negative bids $b_I$, hence change the price from $P(v_I, v_{-I})$ to $P(b_I, v_{-I})$. Define the \emph{incentive-awareness measure}:
$$\delta_I(v_I, v_{-I}) = 1 - \frac{\inf_{b_I\in\mathbb{R}_+^m} P(b_I, v_{-I})}{P(v_I, v_{-I})}, $$
and \emph{interim incentive-awareness measures}: 
\[\delta_{m}^{\interim}(v_{-I}) = \sup_{v_I\in\mathbb{R}_+^m}[ \delta_I(v_I, v_{-I})],\quad\quad\quad\quad\Delta_{N, m}^{\interim} = \E_{v_{-I}\sim F}[ \delta_m^{\interim}(v_{-I})].\]
\end{definition}

Intuitively, the incentive-awareness measure $\Delta_{N, m}^{\interim}$ quantifies the sensitivity of a specific price learning function $P$ to a change of at most $m$ samples out of the $N$ samples. This can be viewed as a measure for the incentive-awareness of $P$, since such changes can be strategically used by a bidder to reduce the resulting reserve price and hence increase the bidder's utility.

\noindent
{\bf Distribution classes. }
%\paragraph{Distribution classes.}
We consider two distribution classes: the class of Monotone Hazard Rate (MHR) distributions (where $\frac{f(v)}{1-F(v)}$ is non-decreasing over the support of the cumulative distribution $F$),
and the class of bounded distributions which consists of all distributions with support included in $[1, D]$.\footnote{The MHR distributions we consider are continuous. The bounded distributions can have mass points.}


\noindent
{\bf Upper bound on incentive-awareness measure for ERM}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Upper bound of Incentive-Awareness Measure for ERM}\label{sec:discount-ratio-definition}

\noindent The main technical part of our paper will therefore focus on analyzing the incentive-awareness measure. We obtain the following main result:

\begin{theorem}\label{thm:discount_combined}
Let $P=\erm^c$. The interim incentive-awareness measure is bounded by
\begin{itemize} 
    \item for MHR $F$, 
    $\Delta^{\interim}_{N, m}=O\left(m\frac{\log^3 N} {\sqrt{N}}\right)$
    , if $m=o(\sqrt{N})$ and $\frac{m}{N}\le c\le\cupperboundmhr$.\footnote{We use $a(n)=o(b(n))$ to denote $\lim_{n\to+\infty}\frac{a(n)}{b(n)}=0$.}
    \item for bounded $F$, $\Delta^{\interim}_{N, m} = O\left(D^{8/3}m^{2/3}\frac{\log^2 N} {N^{1/3}}\right)$, if $m=o(\sqrt{N})$ and  $\frac{m}{N}\le c\le \frac{1}{2D}$. 
\end{itemize}

The constants in the two big $O$'s are independent of $F$ and $c$. 
\end{theorem}

\noindent
The proof of this theorem is further discussed in Section~\ref{sec:discount_ratio_upper-bound}. See Section~\ref{sec:discussion-lower-bound} for a discussion on the tightness of this result.


==> table_comparison.tex <==

\section{Temporary section}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\caption{Comparisons with Online Learning Algorithms Using Differential Privacy}
\label{table:comparison}
\begin{tabular}{@{}llll@{}}
\toprule
                   & \citet{liu2018learning}             & \citet{NIPS2019_abernethy_learning}                                          & Two-phase ERM                                                           \\ \midrule
Distribution       & $[0, D]$                                                                                               & $[0, D]$                                                                                                                 & $[1, D]$                                                                                         \\
\begin{tabular}[c]{@{}l@{}}Revenue (compared\\ to Myerson)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}$\tilde O(D\sqrt[4]{\frac{\overline{m}}{T}})$\\ additive\end{tabular} & \begin{tabular}[c]{@{}l@{}}$\tilde O(\frac{D}{\sqrt{T}})$\\ additive\end{tabular}  & \begin{tabular}[c]{@{}l@{}}$\tilde O(\sqrt[3]{\frac{D}{T}})$\\ multiplicative\end{tabular} \\
Truthfulness       & in equilibrium                                                                                         & $\tilde O(\frac{D\overline{m}}{\sqrt{T}})$                                        & $\tilde O(D^{\frac{11}{3}}\overline{m}^{\frac{5}{3}} T^{-\frac{2}{9}})$                          \\
Total running time & $\Omega(T^{\frac{5}{4}})$                                                                              & $\Omega(T^{\frac{3}{2}})$                                                                                                                                  & $O(T)$                                                                                           \\ 
Input to algorithm & $D$, $T$, bids                                                                                         & $D$, $T$, bids                                                                                                                               & $\overline{m}$, $T$, bids                                                                        \\
Algorithm type     & randomized                                                                                             & randomized                                                                                                                                              & deterministic                                                                                    \\ \bottomrule
\end{tabular}
\end{table}

